Evidence-Inference Reconstruction: When The Evidence Is Recalled But The Reasoning Goes Wrong

Modern multi-hop LLM agents are equipped with built-in mechanisms to detect errors in intermediate reasoning steps. Such errors trigger corrective actions from these agents, which mostly follow the paradigm of retrying the steps or the reasoning trajectories. Not only are these retries expensive, we present in this paper that they are also potentially unnecessary. To this end, we introduce Evidence-Inference Reconstruction (EIR), which uses structured state to guide one retrieval trajectory, accumulating source evidence in the process. We show that as long as the relevant evidence has been collected, EIR is capable of generating the correct answer in a single final model call even if erroneous evidence has been mixed in due to incorrect intermediate reasoning steps. In one evaluation, using Haiku 4.5 and GPT-4.1 Mini, we evaluate EIR on matched 1,000-question subsets of HotpotQA, 2WikiMultiHopQA, and MuSiQue, showing that EIR improves Answer F1, the overlap between the model's and the correct answer, over the baseline by 8.3--32.8 points, Agentic SSR by 10.6--29.1 points, and Reflexion by 1.1--15.9 points. Additionally, we show that EIR averages 4.85 total model calls per question, compared with 35.29 for Agentic SSR and 12.41 for Reflexion. Together, these results corroborate EIR's central premise: separating evidence retrieval from the final answer model call can improve answer accuracy while utilizing substantially less computation.

==> figures/paper/performance_comparison.tex <==
% Requires \usepackage{booktabs}
% Requires \usepackage{graphicx}

\begin{table}[!t]
\centering

\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrr}
\toprule
Method
& Calls/q
& Call range
& Calls/EIR
& \$/q
& \$/EIR
& Answer F1 (\%) \\
\midrule

EIR
& 4.85
& 4.08--5.32
& $1.00\times$
& 0.00738
& $1.00\times$
& 66.89 \\

Agentic SSR
& 35.29
& 30.35--40.30
& $7.28\times$
& 0.02681
& $3.63\times$
& 47.52 \\

Oracle-stopped Reflexion$^\dagger$
& 12.41
& 10.90--14.15
& $2.56\times$
& 0.01149--0.01274
& $1.56$--$1.73\times$
& 58.56 \\

Direct
& 3.24
& 2.78--3.68
& $0.67\times$
& 0.00311
& $0.42\times$
& 47.93 \\

\bottomrule
\end{tabular}%
}

\caption{\textbf{Logical model-call and monetary efficiency with answer quality, averaged across GPT-4.1-mini and Claude Haiku 4.5 on HotpotQA, 2WikiMultiHopQA, and MuSiQue.} Values are unweighted means across six model--benchmark cells, with 1,000 matched questions per cell.}
\label{tab:computation}

\vspace{2pt}

\begin{minipage}{\textwidth}
\footnotesize
Calls are logical model generations excluding provider retries. Call ranges are minimum and maximum cell-level means; call ratios do not measure FLOPs or latency. Monetary costs are reconstructed from audited, persisted provider token accounting using the paper's fixed input/output prices per million tokens: GPT-4.1-mini, \$0.40/\$1.60; Claude Haiku 4.5, \$1.00/\$5.00. They exclude unrecorded retry charges and are not invoice totals. Both ratio columns divide six-cell means by the corresponding EIR mean.

$^\dagger$Reflexion uses gold-answer Exact Match for oracle stopping. Its monetary interval is an accounting bound, not a confidence interval: GPT-4.1-mini records retain trial input/output counts but only total tokens for inter-trial reflections. Following the existing bound convention, the lower endpoint omits those residual tokens and the upper endpoint prices them entirely as output. Haiku's complete episode-level provider input/output counts are used at both endpoints.
\end{minipage}

\end{table}
